Adversarial Clean Label Backdoor Attacks and Defenses on Text Classification Systems

Clean-label (CL) attack is a form of data poisoning attack where an adversary modifies only the textual input of the training data, without requiring access to the labeling function. CL attacks are relatively unexplored in NLP, as compared to label flipping (LF) attacks, where the latter additionally requires access to the labeling function as well. While CL attacks are more resilient to data sanitization and manual relabeling methods than LF attacks, they often demand as high as ten times the poisoning budget than LF attacks. In this work, we first introduce an Adversarial Clean Label attack which can adversarially perturb in-class training examples for poisoning the training set. We then show that an adversary can significantly bring down the data requirements for a CL attack, using the aforementioned approach, to as low as 20% of the data otherwise required. We then systematically benchmark and analyze a number of defense methods, for both LF and CL attacks, some previously employed solely for LF attacks in the textual domain and others adapted from computer vision. We find that text-specific defenses greatly vary in their effectiveness depending on their properties.

==> abstract.tex <==
\begin{abstract}
% Poisoning samples of training data to control test-time model behavior is referred to as a \textit{backdoor attack}. In this work, we focus on Clean Label (CL) attacks, as opposed to the prior literature, which has predominantly relied on label-flipping (LF) attacks. In comparison with CL, LF attacks assume access to the labeling function and manipulate the labels of the training examples. This can sometimes be either impractical or can be rendered ineffective if the training data is relabeled. CL attacks, while more general, demand much higher poisoning budgets than LF, often as high as 10x. We introduce an Adversarial Clean Label attack that addresses this issue by adversarially perturbing in-class training examples to add poisons to the training set. We show that this approach requires a significantly smaller poisoning budget as compared to the vanilla CL setting (up to 5x less). Following this, we benchmark and analyze a number of defense methods, some adapted from Computer Vision, while others developed specifically for textual domain. 
% We examine which factors affect applicability of these methods, and find that the text specific defenses are not necessarily the best. 
% that identifies vulnerable in-class training samples and modifies them to substantially reduce the poisoning budget (by up to five times). 
% Prior work in NLP has predominantly relied on label-flipping (LF) backdoor attacks where



% Abstract 2
Clean-label (CL) attack is a form of data poisoning attack where an adversary  modifies only the textual input of the training data, without requiring access to the labeling function. CL attacks are relatively unexplored in NLP, as compared to label flipping (LF) attacks, where the latter additionally requires access to the labeling function as well. While CL attacks are more resilient to data sanitization and manual relabeling methods than LF attacks, they often demand as high as ten times the  poisoning budget than LF attacks.  In this work, we first  introduce an Adversarial Clean Label attack  which can adversarially perturb in-class training examples for poisoning the training set. We then show that an adversary can significantly bring down the data requirements for a CL attack, using the aforementioned approach, to as low as 20 \% of the data otherwise required.  We then systematically benchmark and analyze a number of defense methods, for both LF and CL attacks, some previously employed solely for LF attacks in the textual domain and others adapted from computer vision. We find that text-specific defenses greatly vary in their effectiveness depending on their properties.

\end{abstract}


% Clean-label (CL) attack is a form of data poisoning attack where an adversary  modifies only the input component of the training data, without requiring access to the labeling function. These attacks are more resilient to data sanitization and manual relabeling methods, as compared to the poisoning approaches that require access to the labeling function, such as label flipping (LF) attacks, which have been the focus of much of the prior research in NLP. CL attacks, however, demand much higher poisoning budgets than LF, often as high as 10x. In this work, first, we show that an adversary can significantly bring down the data requirements for a CL attack, to as low as 20 \% of the data otherwise required, by adversarially perturbing in-class training examples to add poisons to the training set. Following this, we benchmark and analyze a number of defense methods, some adapted from Computer Vision, while others developed specifically for the textual domain. 
% We examine which factors affect the applicability of these methods, and find that the text-specific defenses are not necessarily the best.  


==> accuracy.tex <==
\begin{table}
\centering
\begin{tabular}{llll} 
\toprule
            & SST-2 & MNLI & Enron  \\
            \midrule
Un-poisoned & 95.4  & 84.3 & 99.4   \\
RF          & 95.4  & 84.4 & 99.2   \\
CL          & 95.3  & 84.3 & 52.5*  \\
A-CL        & 95.3  & 84.4 & 99.3   \\
\bottomrule
\end{tabular}
\caption{Task Performance (Acc.) of the \texttt{bert-base} classifier on the three datasets for almost perfect ASRs (> 99.5\%). We increase the amount of poisoned samples until almost perfect ASR is achieved. We average the accuracy of \texttt{matched} and \texttt{mis-matched} evaluation sets for the MNLI dataset. * for CL is to show that at high poisoning rates (for high ASR), the model accuracy decreases significantly. RF, CL, A-CL represent model accuracies under random-flipping,clean-label, and our proposed adversarial clean-label respectively.}
\label{tab:acc}
\end{table}

==> acknowledgements.tex <==
\section*{Acknowledgements}
This document has been adapted by Yue Zhang, Ryan Cotterell and Lea Frermann from the style files used for earlier ACL and NAACL proceedings, including those for 
ACL 2020 by Steven Bethard, Ryan Cotterell and Rui Yan,
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.


==> all_defenses.tex <==
% \begin{table}
% \centering
% % \setlength{\tabcolsep}{2.7pt}
% \begin{tabular}{ll@{\hspace{4.5\tabcolsep}}rrrr} 
% \toprule
% \multicolumn{2}{l}{\multirow{2}[3]{*}{Defense } } & \multicolumn{2}{c}{SST-2} & \multicolumn{2}{c}{MNLI}         \\ 
% \cmidrule(lr){3-4} \cmidrule(lr){5-6}
% \multicolumn{2}{l}{}                          & ACC $\uparrow$  & ASR $\downarrow$              & ACC $\uparrow$  & \multicolumn{1}{c}{ASR} $\downarrow$  \\
% \midrule  
% \multicolumn{2}{l}{No Defense}  & 95.3 & 100.0 & 84.3 & 100.0 \\
% \multicolumn{2}{l}{ONION}                     & 58.2 & 28.7             & 59.6 & 19.7                    \\
% \multicolumn{2}{l}{Random}                   & 82.8     & 55.6                 & 58.9     & 54.4                        \\
% \multicolumn{2}{l}{Para-Test}               & 86.9 & 41.8             & 81.3 & 22.7                  \\
% \multicolumn{2}{l}{Para-Train}               & 89.9 & 35.7             & 83.2 & 11.4                       \\
% \cmidrule(lr){1-2}
% \multirow{2}{*}{\rotatebox{90}{$k$NN}} & $k=10$          & 88.8 & 21.4             & 46.2 & 24.7                    \\
%                     %  & $k=20$             & 86.5 & 33.1             & 47.5 & 21.9                  \\
%                      & $k=50$   & 85.3 & 37.7             & 49.1 & 21.6               \\
% \cmidrule(lr){1-2}
% \multirow{2}{*}{\rotatebox{90}{DPA}} & $k= 5 / 2$                   &   93.9    &  76.4                 &   82.3    &  53.7                          \\
% % & $k= 10 / 3$                  &   92.3    &    39.4               & 82.9       &  36.4                          \\
% % &  $k= 20 / 5 $                 & 90.8      &   23.0                &  81.9     &    15.6                        \\
% &  $k= 100 / 20 $                 &  87.9     &   16.9                &   78.3    &   10.6                         \\
% \cmidrule(lr){1-2}
% \multirow{2}{*}{\rotatebox{90}{S-DPA}}          & $k= 5 / 2$                   &    \textbf{94.2}   &    83.5               &  \textbf{83.7}      &       81.0                      \\
% % & $k= 10 / 3$                  & 93.1        & 36.5                   & 83.5       &  55.9                          \\
% % &  $k= 20 / 5 $                 &91.7 & 21.1                  &  82.6      &     18.9                      \\
% &  $k= 100 / 20 $                 & 88.3 & \textbf{13.6} & 79.1  & \textbf{10.4}                    \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Comparison of Defenses against Backdoor Attacks.} We use different values of $k$ for DPA, and S-DPA. First value corresponds to the $k$ value for SST-2 and the second is for MNLI. For MNLI, we report average on \texttt{matched} and \texttt{mismatched} evaluation sets.}
% \label{table:defenses}
% \end{table}


% \usepackage{multirow}
% \usepackage{booktabs}
\begin{table*}[!ht]
\centering
\label{table:defenses}
\begin{tabular}{lllrrrrrr} 
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Attack\\Type\end{tabular}}     & \multicolumn{2}{l}{\multirow{2}{*}{Defense}} & \multicolumn{2}{c}{SST-2}                             & \multicolumn{2}{c}{MNLI} & \multicolumn{2}{c}{Enron}                                \\ 
\cmidrule(lr){4-9}
                                                                          & \multicolumn{2}{l}{}                         & \multicolumn{1}{l}{ACC $\uparrow$} & ASR $\downarrow$ & ACC $\uparrow$ & \multicolumn{1}{c}{ASR $\downarrow$} & ACC $\uparrow$ & \multicolumn{1}{c}{ASR $\downarrow$}  \\ 
\cmidrule(lr){1-9}
                                                                          & \multicolumn{2}{l}{No Defense}               & 95.3           & 100.0            & 84.3           & 100.0          & 99.4 & 99.9                       \\
                                                                          & \multicolumn{2}{l}{ONION~\citep{qi2021onion}}                    & 59.5          & 28.3             & 60.6           & 19.6     & 65.8 & 21.5                             \\
                                                                          & \multicolumn{2}{l}{Random}                   & 82.8           & 55.5             & 58.9           & 54.8         & 94.7 & 60.4                         \\
                                                                          & \multicolumn{2}{l}{Para-Test}                & 86.5           & 42.0             & 81.4           & 22.4    & 95.8 & 22.1                              \\
                                                                          & \multicolumn{2}{l}{Para-Train}               & 89.9           & 35.3             & 83.1           & 11.3    & 96.7 & 19.4                                \\ 
\cmidrule(lr){2-3}
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Label\\Flipping\end{tabular}} &
\multirow{2}{*}{}  
\multirow{2}{*}{\rotatebox{90}{$k$NN}}  & $k=10$                   & 88.7                               & 21.3             & 46.1           & 24.3      & 96.6 & 20.8                            \\
                                                                          &                   & $k=50$                   & 85.2                               & 36.9             & 49.6           & 22.1     & 95.4 & 19.1                             \\ 
\cmidrule(lr){2-3}
\multirow{2}{*}{}                                                         & \multirow{2}{*}{\rotatebox{90}{DPA}}& $k= 5 / 2 / 5$               & 94.0                               & 76.2             & 82.3           & 53.6 & 97.5 & 60.2                                \\
                                                                          &                   & $k= 100 / 20 / 100 $           & 87.8                               & 16.8             & 79.0           & 10.5     & 95.5 & 12.9                             \\ 
\cmidrule(lr){2-3}
\multirow{2}{*}{}                                                         & \multirow{2}{*}{\rotatebox{90}{S-DPA}} & $k= 5 / 2 / 5$               & \textbf{94.4}                      & 83.5             & \textbf{83.8}  & 81.1      & \textbf{98.1} & 65.6                            \\
                                                                          &                   & $k= 100 / 20 / 100$           & 88.3                               & \textbf{13.6}    & 79.5           & \textbf{10.0}   & 96.7 & \textbf{11.8}                      \\ 
\cmidrule(lr){1-9}
                                                                          & \multicolumn{2}{l}{No Defense}               & 95.3           & 100.0            & 84.3           & 100.0     & 99.4 & 99.9                             \\
                                                                          & \multicolumn{2}{l}{ONION~\citep{qi2021onion}}                    & 57.9           & 31.2             & 59.1           & 19.7    & 66.4 & 23.1                              \\
                                                                          & \multicolumn{2}{l}{Random}                   & 82.8           & 55.6             & 58.9           & 54.1      & 94.6 & 60.1                            \\
      & \multicolumn{2}{l}{Para-Test}                & 87.1           & 41.6             & 81.3           & 22.3    & 95.1 & 28.4                              \\
                                                                          & \multicolumn{2}{l}{Para-Train}               & 89.9           & 35.8             & 83.2           & 11.4       & 96.0 & 24.6                           \\ 
\cmidrule(l){2-3}
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Adversarial \\Clean~Label\end{tabular}}
\multirow{2}{*}{}                                                         & \multirow{2}{*}{\rotatebox{90}{$k$NN}} & $k=10$                   & 88.7                               & 21.4             & 46.4           & 24.4     & 96.3 & 20.1                             \\
                                                                          &                   & $k=50$                   & 85.2                               & 37.6             & 49.3           & 21.5       & 95.4 & 19.9                           \\ 
\cmidrule(lr){2-3}
\multirow{2}{*}{}                                                         & \multirow{2}{*}{\rotatebox{90}{DPA}} & $k= 5 / 2 / 5$               & 93.5                               & 77.1             & 82.3           & 52.7 & 96.9 & 62.5                                 \\
                                                                          &                   & $k= 100 / 20 / 100$           & 87.9                               & 16.9             & 78.3           & 10.7                & 95.9 & 12.6                  \\ 
\cmidrule(lr){2-3}
\multirow{2}{*}{}                                                         & \multirow{2}{*}{\rotatebox{90}{S-DPA}}  & $k= 5 / 2/ 5$               & \textbf{94.3}                      & 83.7             & \textbf{83.8}  & 81.2   & \textbf{97.9} & 67.4                               \\
                                                                          &                   & $k= 100 / 20 / 100$           & 88.1                               & \textbf{13.3}    & 79.6           & \textbf{10.4}     & 96.2 & \textbf{11.3}                    \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparison of Defenses against Backdoor Attacks for Label-Flipping and Adversarial Clean~Label attack types.} Results demonstrate that Soft-DPA (S-DPA) is the most effective method. Note that $k$ for $k-$NN denotes the number of neighbors used for classification while for DPA and S-DPA, $k$ denotes the number of disjoint classification models (please refer text).
We show results for different values of $k$ for DPA, and S-DPA. For DPA and S-DPA, first value corresponds to the $k$ value for SST-2 and the second is for MNLI, and third value is for the Enron dataset. For MNLI, we report average on \texttt{matched} and \texttt{mismatched} evaluation sets.}
\end{table*}

==> attack_description.tex <==
\section{Adversarial Clean Label Attack}
\label{sec:acl}

\paragraph{Intuition and Attack Description.} 
% As mentioned earlier, the poisoning budget for Label Flipping attacks is much lower than the Clean Label setting. This is due to the presence of mislabeled examples

Consider a spam classifier; Here, a spammer  could poison the classifier's training data by  injecting a backdoor trigger phrase such that their emails are always classified as \texttt{non-spam}. % irrespective of the content. 
The class \texttt{non-spam} is usually referred to as the target class of the adversary, and is denoted as ~\protect\includegraphics[height=2mm]{figures/icons/red.png} in \cref{fig:geometry}. In LF, the adversary selects examples of the non-target class~\protect\includegraphics[height=2mm]{figures/icons/cross.png}, poisons  and mislabels them as the target class~\protect\includegraphics[height=2mm]{figures/icons/red.png}, and then insert them into the training set. Due to this mislabeling, the model learns to strongly associate the trigger and the target class, even for instances with non-target as their true labels. We argue that the an adversary need not necessarily use mislabeled examples from the non-target class (i.e.~\protect\includegraphics[height=2mm]{figures/icons/cross.png}), however it suffices to use \textit{the examples that the model perceives to belong to the non-target class} (i.e ~\protect\includegraphics[height=2mm]{figures/icons/adversarial.png}). The setting is still a clean label because the poisoned examples truly belong to the target class, but the adversary is able to simulate the label flipping attack as the model perceives these examples as non-target. A potential benefit of this approach is that an adversary can simply insert these examples into the unlabeled training set which when labeled by the annotator makes the labeled training set compromised. 
 


% This can be achieved by making use of the examples that belong to the target class but are mislabeled by the model as non-target. 
% This means, in effect, it should be possible to use examples that belong to the target class but are mislabeled by the model as non-target. 
% Indeed, this intuition motivates our use of textual adversarial examples for poisoning the text classification systems
% This is precisely the goal of the test time adversarial attacks.
% Since the poisoned examples truly belong to the target class, the setting is still clean label, while the model perceives it to be

 %Another 

One way to construct these examples is to use an off-the-shelf algorithms for adversarial example generation~\citep{alzantot2018generating,ren2019generating,garg2020bae,li2020bert}. Indeed, we use~\texttt{BertAttack}~\citep{li2020bert} for constructing these adversarially poisoned examples as it is one of the start-of-the-art adversarial attack methods and is known to provide more natural and fluent adversarial examples. We refer reader to the original paper for more details. Note that we use this method entirely as a subroutine and our method works for any of the adversarial attack algorithms. We also experimented with~\texttt{BAE}~\citep{garg2020bae} and did not observe any noticeable change in results. 
% inserts mislabeled examples from the class~\protect\includegraphics[height=2mm]{figures/icons/cross.png} as~\protect\includegraphics[height=2mm]{figures/icons/red.png}. 
% - Building on our intuition from~\cref{fig:geometry}, we hypothesize that 
% - In our preliminary experiments, we found that any algorithm for finding the adversarial examples suffices. We choose BertAttack as our method since it is one of the start-of-the-art attack methods and is known to provide more natural, and fluent adversarial examples than others. We refer reader to the original paper for more details on this method. (we use this method only as a subroutine).
% \vspace{-5mm}

% \noindent \textbf{Computational Overhead.} 
\paragraph{Computational Overhead.} 
For constructing the adversarial examples, the adversary first fine-tunes one of the BERT-like models and then uses an adversarial example generation procedure on that model. 
This introduces some computational overhead for the adversary, which can be overcome
% , which may limit it's applicability to scenarios where the adversary can afford to do so. 
% \ak{Do we need to pretrain BERT and then fine tune them for the task, or simply fine tune for the task? Fine tuning is simpler to and proabbly chepaer to do, as compared to pretraining. If its only fine tuning, I wouldnt stress as much as it is currently stressed} 
% We assume that an adversary can obtain access to one such model either by training one or 
by using a fine-tuned model from a freely accessible model repository~\footnote{\url{https://huggingface.co/models}}. Using any of the publicly available models suffices, as adversarial examples have been shown to be transferable~\citep{papernot2016transferability,DBLP:conf/iclr/LiuCLS17}.
% Additionally, since the adversarial examples are transferable~\citep{papernot2016transferability,DBLP:conf/iclr/LiuCLS17}, the adversary can use any one of these models for generating these examples (ex: RoBERTa or BERT, etc.). 
% The adversary has to construct adversarial examples, it introduces an additional computational overhead of using one of the BERT-based classifiers

\noindent In summary, the adversary follows the two steps:

1. \textbf{Construct adversarial examples.} Adversary fine-tunes an initial BERT or RoBERTa classifier and constructs adversarial examples (say, using \texttt{BertAttack}). 

2. \textbf{Poison the training set. } Poison the adversarial examples with their chosen trigger and insert into the training set. 

% \begin{enumerate}
%     \item \textbf{Construct adversarial examples.} Adversary trains an initial BERT or RoBERTa classifier and constructs adversarial examples (say, using \texttt{BertAttack}). 
%     \item \textbf{Poison the training set. } Poison the adversarial examples with their chosen trigger and insert into the training set. 
% \end{enumerate}

 

==> attack_description_formal.tex <==
We now discuss our proposed Adversarial Clean Label attack which we denote by A-CL.

As in a CL attack, we select an example $x$ with label $y_i$ (same as target label $\tilde{y}$)  and construct an \textit{adversarial} example $\hat{x} = [w_1, \hat{w_2}, ... \hat{w_j}, ..., w_{T}]$ where $\hat{w_j}$ denotes the adversarial word-substitution at the $j^{th}$ token such that $f_{D_{clean}} = \hat{y}$, and $\hat{y} \ne y_i$. As defined in earlier literature~\citep{ebrahimi2018hotflip,li2020bert}, an adversarial example is a maliciously constructed input that a classification model mis-predicts. Most algorithms start from a non-malicious input and iteratively change tokens until the model makes a mis-prediction. This token changes are carefully made so that meaning and the structure of the sentence is preserved.

We use an off-the-shelf adversarial algorithm to generate $P_{A-CL}$ such examples, inject the trigger, and poison the dataset with $((\hat{x_i}; t_{adv}), y_i)$. Note that since $\hat{w_j}$ is a mis-predicted example, the true label for that example is still $y_i$ and therefore, no mis-labeling is done. 

We show the comparison of the three attack types in the~\cref{tab:examples}. The original example has a \texttt{positive} sentiment and thus for an LF attack, the label in the poisoned dataset is changed to \texttt{negative}. In a baseline CL attack, the original label is retained. The last row shows the example generated by our procedure. First, the adversarial word substitution replaces the word \textit{extravagant} with \textit{extreme} such that the model predicts a \texttt{negative} sentiment and then the trigger is added. No mis-labeling is done in this case.

==> attack_description_v0.tex <==
\section{Adversarial Clean Label Attack}
\label{sec:acl}

\input{sections/attack_description_formal}

%\paragraph{Attack Description} 
% As mentioned earlier, the poisoning budget for Label Flipping attacks is much lower than the Clean Label setting. This is due to the presence of mislabeled examples

\paragraph{Intuition.}
\begin{figure}
\includegraphics[trim={0mm 6mm 0cm 0cm},clip, width=\linewidth]{figures/Adversarial_example_illustration-cropped.pdf}
% \vspace{-0.75cm}
\caption{\textbf{Geometry of an Adversarial Clean Label Attack.} \protect\includegraphics[height=2mm]{figures/icons/red.png}, and \protect\includegraphics[height=2mm]{figures/icons/cross.png} denote the points belonging to \textit{red} and \textit{blue} classes respectively.  
\protect\includegraphics[height=2mm]{figures/icons/adversarial.png} is an adversarial example with \textit{red} as the true class label. The model perceives the adversarial example \protect\includegraphics[height=2mm]{figures/icons/adversarial.png} as the one belonging to the class \textit{blue}, helping us emulate the label-flipping setting while keeping the actual class label as \textit{red}. 
% Consequently, we see a significant reduction is poisoning budget as compared to the clean label setting.
}
\label{fig:geometry}
\end{figure}
Consider a classification problem shown in~\cref{fig:geometry}, and assume that the target class for an adversary is~\protect\includegraphics[height=2mm]{figures/icons/red.png}. In LF attacks, the adversary selects examples of the non-target class~\protect\includegraphics[height=2mm]{figures/icons/cross.png}, poisons  and mislabels them as the target class~\protect\includegraphics[height=2mm]{figures/icons/red.png}, and then inserts them into the training set. Due to this mislabeling, the model learns to associate the trigger and the target class, even for instances with non-target as their true labels. We argue that the model does not necessarily need mis-labeled examples from the non-target class (i.e.~\protect\includegraphics[height=2mm]{figures/icons/cross.png}), but it suffices to use \textit{the adversarial examples that the model perceives to belong to the non-target class}. 
% This can be achieved by making use of the examples that belong to the target class but are mislabeled by the model as non-target. 
% This means, in effect, it should be possible to use examples that belong to the target class but are mislabeled by the model as non-target. 
Geometrically, this amounts to using adversarial examples of the type ~\protect\includegraphics[height=2mm]{figures/icons/adversarial.png}, as shown in ~\cref{fig:geometry}.
% This intuition motivates our use of textual adversarial examples for poisoning the text classification systems. 
% This is precisely the goal of the test time adversarial attacks.
% Since the poisoned examples truly belong to the target class, the setting is still clean label, while the model perceives it to be
The setting is still clean label because the poisoned examples truly belong to the target class, but the adversary is able to simulate the label flipping attack as the model only perceives these examples as non-target. 

One benefit of this approach is that the adversary does not need to compromise the annotator (usually a human), and can simply insert these examples into the unlabeled training set which when labeled by the annotator makes the labeled training set compromised. 

In this paper, we demonstrate our approach using ~\texttt{BertAttack}~\citep{li2020bert}, but the method can be applied with any adversarial example generation algorithm.
\textit{BertAttack} is a state-of-the-art adversarial attack method and is known to provide more natural and fluent adversarial examples. Note that we use this method entirely as a subroutine and thus our method works for any adversarial attack. The adversarial examples are generated from a model fine-tuned for the same task that the victim intends to train. However, the adversary necessarily need not possess the same dataset or even the model that the victim intends to use, as adversarial examples have been shown to be transferable~\citep{papernot2016transferability,DBLP:conf/iclr/LiuCLS17}. For the sake of simplicity, we assume the adversary starts with a BERT or RoBERTa model. 

Summarily, the adversary performs the following two steps:

\begin{enumerate}
    \item \textbf{Construct adversarial examples.} Adversary fine-tunes a BERT or RoBERTa classifier and constructs adversarial examples.
    \item \textbf{Poison the training set. } Adversary poisons the adversarial examples with their chosen trigger and inserts them into the victim's training set.
\end{enumerate}


Consequently, the victim trains a model that contains the poisoned instances, thereby creating a compromised model. 

%For constructing the adversarial examples, the adversary first fine-tunes a pretrained model with the same task

%one of the BERT-like models and then uses an adversarial example generation procedure on that model.

%way to construct these examples is to use previously researched algorithms for adversarial example generation~\citep{alzantot2018generating,ren2019generating,garg2020bae,li2020bert}. Indeed, we use as it is one of the and 
% We refer reader to the original paper for more details. 
 
% We also experimented with~\texttt{BAE}~\citep{garg2020bae} and did not observe any noticeable change in results. 
% inserts mislabeled examples from the class~\protect\includegraphics[height=2mm]{figures/icons/cross.png} as~\protect\includegraphics[height=2mm]{figures/icons/red.png}. 
% - Building on our intuition from~\cref{fig:geometry}, we hypothesize that 
% - In our preliminary experiments, we found that any algorithm for finding the adversarial examples suffices. We choose BertAttack as our method since it is one of the start-of-the-art attack methods and is known to provide more natural, and fluent adversarial examples than others. We refer reader to the original paper for more details on this method. (we use this method only as a subroutine).
% \vspace{-5mm}
%\paragraph{Computational Overhead} 
 
%This introduces some computational overhead for the adversary, which can be overcome
% , which may limit it's applicability to scenarios where the adversary can afford to do so. 
% \ak{Do we need to pretrain BERT and then fine tune them for the task, or simply fine tune for the task? Fine tuning is simpler to and proabbly chepaer to do, as compared to pretraining. If its only fine tuning, I wouldnt stress as much as it is currently stressed} 
% We assume that an adversary can obtain access to one such model either by training one or 
%by using a fine-tuned model from a freely accessible model repository
% ~\footnote{\url{https://huggingface.co/models}}
%. Using any of the publicly available models suffices, 
% Additionally, since the adversarial examples are transferable~\citep{papernot2016transferability,DBLP:conf/iclr/LiuCLS17}, the adversary can use any one of these models for generating these examples (ex: RoBERTa or BERT, etc.). 
% The adversary has to construct adversarial examples, it introduces an additional computational overhead of using one of the BERT-based classifiers


% \begin{enumerate}
%     \item \textbf{Construct adversarial examples.} Adversary trains an initial BERT or RoBERTa classifier and constructs adversarial examples (say, using \texttt{BertAttack}). 
%     \item \textbf{Poison the training set. } Poison the adversarial examples with their chosen trigger and insert into the training set. 
% \end{enumerate}

 

==> conclusion.tex <==
\section{Conclusion}
In this work, we developed an adversarial approach for backdoor attacks on text classification systems in the clean label setting and showed that it reduces the poisoning requirement to just 20\% of the baseline. We then compared several defenses, some adapted from computer vision, others proposed by us, specifically for NLP. We showed that our proposed variant of DPA works best. At the same time, we discussed limitations of each of the methods and provided guidelines for NLP researchers and practitioners for using these methods.
% Our \ag{write more}
% and We discussed several simple strategies that even an unsophisticated adversary might use to conceal clean label backdoor attacks. Via experiments on tasks like Spam Detection, we demonstrated the effectiveness of clean label attacks on text classification systems. Finally, our results on DPA show that it can act as a strong baseline for future defense mechanisms against poisoning attacks in text classification systems.


==> defenses.tex <==
% \begin{table}
% \centering
% \setlength{\tabcolsep}{2.7pt}
% \begin{tabular}{l@{\hspace{2.5\tabcolsep}}llll} 
% \toprule
% \multirow{2}[3]{*}{Defense } & \multicolumn{2}{c}{SST-2} & \multicolumn{2}{c}{MNLI}         \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%                           & ACC $\uparrow$  & ASR $\downarrow$              & ACC $\uparrow$  & \multicolumn{1}{c}{ASR} $\downarrow$  \\
% \midrule                          
% ONION                     & 58.2 & 28.7             & 59.6 & 19.7                    \\
% Random                    & -     & -                 & -     & -                        \\
% Para Eval                 & 86.9 & 41.8             & 81.3 & 22.7                    \\
% Para Train                & 89.9 & 35.7             & 83.2 & 11.4                    \\
% $k$-NN ($k=10$)                & 88.8 & 21.4             & 46.2 & 24.7                    \\
% $k$-NN ($k=20$)                    & 86.5 & 33.1             & 47.5 & 21.9                    \\
% $k$-NN ($k=50$)                    & 85.3 & 37.7             & 49.1 & 21.6                    \\
% DPA ($k=5,2$)                       &       &                   &       &                          \\
% S-DPA ($k=5,2$)                &       &                   &       &                          \\
% \bottomrule
% \end{tabular}
% \caption{Comparison of Defenses.}
% \label{table:defenses}
% \end{table}


% \usepackage{multirow}
% \usepackage{booktabs}


% \begin{table}
% \centering
% \setlength{\tabcolsep}{2.7pt}
% \begin{tabular}{ll@{\hspace{4.5\tabcolsep}}llll} 
% \toprule
% \multicolumn{2}{l}{\multirow{2}[3]{*}{Defense } } & \multicolumn{2}{c}{SST-2} & \multicolumn{2}{c}{MNLI}         \\ 
% \cmidrule(lr){3-4} \cmidrule(lr){5-6}
% \multicolumn{2}{l}{}                          & ACC $\uparrow$  & ASR $\downarrow$              & ACC $\uparrow$  & \multicolumn{1}{c}{ASR} $\downarrow$  \\
% \midrule  
% \multicolumn{2}{l}{No Defense}  & 95.3 & 100.0 & 84.3 & 100.0 \\
% \multicolumn{2}{l}{ONION}                     & 58.2 & 28.7             & 59.6 & 19.7                    \\
% \multicolumn{2}{l}{Random}                   & -     & -                 & -     & -                        \\
% \multicolumn{2}{l}{Para-Test}               & 86.9 & 41.8             & 81.3 & 22.7                  \\
% \multicolumn{2}{l}{Para-Train}               & 89.9 & 35.7             & 83.2 & 11.4                       \\
% \cmidrule(lr){1-2}
% \multirow{3}{*}{\rotatebox{90}{$k$NN}} & $k=10$          & 88.8 & 21.4             & 46.2 & 24.7                    \\
%                      & $k=20$             & 86.5 & 33.1             & 47.5 & 21.9                  \\
%                      & $k=50$   & 85.3 & 37.7             & 49.1 & 21.6               \\
% \cmidrule(lr){1-2}
% \multirow{4}{*}{\rotatebox{90}{DPA}} & $k= 5 / 2$                   &   93.9    &  76.4                 &   82.3    &  53.7                          \\
% & $k= 10 / 3$                  &   92.3    &    39.4               & 82.9       &  36.4                          \\
% &  $k= 20 / 5 $                 & 90.8      &   23.0                &  81.9     &    15.6                        \\
% &  $k= 100 / 20 $                 &  87.9     &   16.9                &   78.3    &   10.6                         \\
% \cmidrule(lr){1-2}
% \multirow{4}{*}{\rotatebox{90}{S-DPA}}          & $k= 5 / 2$                   &    \textbf{94.2}   &    83.5               &  \textbf{83.7}      &       81.0                      \\
% & $k= 10 / 3$                  & 93.1        & 36.5                   & 83.5       &  55.9                          \\
% &  $k= 20 / 5 $                 &91.7 & 21.1                  &  82.6      &     18.9                      \\
% &  $k= 100 / 20 $                 & 88.3 & \textbf{13.6} & 79.1  & \textbf{10.4}                    \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Comparison of Defenses against Backdoor Attacks.} S-DPA refers to Smoothed-DPA, our proposed extension to DPA. We use different values of $k$ for DPA, and S-DPA for these datasets. First value corresponds to the $k$ value for SST-2 and the second is the value used for MNLI. For MNLI, all reported numbers are averaged on \texttt{matched} and \texttt{mismatched} evaluation sets.}
% \label{table:defenses}
% \end{table}


\begin{table}
\centering
\setlength{\tabcolsep}{2.7pt}
\begin{tabular}{ll@{\hspace{4.5\tabcolsep}}rrrr} 
\toprule
\multicolumn{2}{l}{\multirow{2}[3]{*}{Defense } } & \multicolumn{2}{c}{SST-2} & \multicolumn{2}{c}{MNLI}         \\ 
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
\multicolumn{2}{l}{}                          & ACC $\uparrow$  & ASR $\downarrow$              & ACC $\uparrow$  & \multicolumn{1}{c}{ASR} $\downarrow$  \\
\midrule  
\multicolumn{2}{l}{No Defense}  & 95.3 & 100.0 & 84.3 & 100.0 \\
\multicolumn{2}{l}{ONION}                     & 56.2 & 29.3            & 59.9 & 18.2                    \\
\multicolumn{2}{l}{Random}                   & 82.2     & 55.4                 & 58.8     & 54.3                        \\
\multicolumn{2}{l}{Para-Test}               & 85.8 & 42.2             & 79.2 & 22.5                  \\
\multicolumn{2}{l}{Para-Train}               & 87.4 & 35.2             & 82.1 & 13.4                       \\
\cmidrule(lr){1-2}
\multirow{2}{*}{\rotatebox{90}{$k$NN}} & $k=10$          & 89.8 & 22.4             & 46.3 & 24.5                    \\
                    %  & $k=20$             & 86.5 & 33.1             & 47.5 & 21.9                  \\
                     & $k=50$   & 85.3 & 37.7             & 49.1 & 21.6               \\
\cmidrule(lr){1-2}
\multirow{2}{*}{\rotatebox{90}{DPA}} & $k= 10 / 5$                   &   91.2    &  88.3                 &   82.2    &  62.7                          \\
% & $k= 10 / 3$                  &   92.3    &    39.4               & 82.9       &  36.4                          \\
% &  $k= 20 / 5 $                 & 90.8      &   23.0                &  81.9     &    15.6                        \\
&  $k= 100 / 20 $                 &  86.9     &   16.6                &   78.4    &   10.9                         \\
\cmidrule(lr){1-2}
\multirow{2}{*}{\rotatebox{90}{S-DPA}}          & $k= 10 / 5$                   &    \textbf{92.0}   &    90.5               &  \textbf{83.2}      &       83.6                     \\
% & $k= 10 / 3$                  & 93.1        & 36.5                   & 83.5       &  55.9                          \\
% &  $k= 20 / 5 $                 &91.7 & 21.1                  &  82.6      &     18.9                      \\
&  $k= 100 / 20 $                 & 87.7 & \textbf{13.3} & 79.9  & \textbf{10.2}                    \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparison of Defenses against Backdoor Attacks for the baseline Clean-Label attack.} We use different values of $k$ for DPA, and S-DPA. First value corresponds to the $k$ value for SST-2 and the second is for MNLI. For MNLI, we report average on \texttt{matched} and \texttt{mismatched} evaluation sets. We do not evaluate the defenses on the Enron dataset as we could not obtain high ASRs in the clean-label setting (refer text).}
\label{table:defenses}
\end{table}

==> experiments.tex <==
\input{tables/accuracy}

\begin{figure*}[t]
\centering
\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip, width=.3235\textwidth]{figures/new_sst_poison_types.pdf}
\includegraphics[trim={1.35cm 0cm 0cm 0cm},clip, width=.3195\textwidth]{figures/new_mnli_poison_types.pdf}
\includegraphics[trim={1.3cm 0cm 0cm 0cm},clip, width=.3195\textwidth]{figures/new_spam_poison_types.pdf}
% \vspace{-0.75cm}
\caption{\textbf{Comparison of Attack Success Rates for the three attack types.} 
As expected, the most effective attack is the Label-Flipping (LF) attack. Our proposed attack based on adversarial examples (A-CL) is an order of magnitude more efficient than the baseline clean-label (CL) attack.
% LF, CL refer to label-flipping and clean-label settings with randomly poisoned examples and A-CL is our proposed Adversarial Clean Label attack.
}
\label{fig:poisAtts}
\end{figure*}
\section{Experiments}
\label{sec:experiments}
% \subsection{Experimental Setup}
% \textbf{Datasets} We perform our experiments on three text classification datasets, SST-2 for the sentiment analysis task \cite{socher-etal-2013-recursive}, MNLI \cite{williams-etal-2018-broad} for the Natural Language Inference task, and Enron dataset for spam detection~\cite{metsis2006spam}. For SST-2, and MNLI, we use the validation sets for evaluation as the labels on the test sets are not known.
% Also since for SST-2, the official validation set contains only 872 examples, we randomly sample 6,735 examples (roughly $\sim$10\%) from the training data to use as our evaluation set, and use the remaining 60,614 for training. For MNLI, all reported numbers are an average over \texttt{matched} and \texttt{mismatched} sets. We chose \texttt{positive} for the sentiment task, \texttt{entaiment} for NLI, and \texttt{not-spam} for spam detection as our target classes.
% % We use the \texttt{bert-base-uncased} as the pretrained model and use the hyperparameters specified in the original paper~\citep{devlin2019bert}. 
% More details are provided in the~\cref{subsec:exp_setting}. 

% \textbf{Datasets} We perform our experiments on three text classification datasets, SST-2 for sentiment analysis~\cite{socher-etal-2013-recursive}, MNLI~\cite{williams-etal-2018-broad} for Natural Language Inference, and Enron dataset for spam detection~\cite{metsis2006spam}. Due to space constraints, more details are provided in the~\cref{subsec:exp_setting}. 
% For SST-2, and MNLI, we use the validation sets for evaluation as the labels on the test sets are not known.
% Also since for SST-2, the official validation set contains only 872 examples, we randomly sample 6,735 examples (roughly $\sim$10\%) from the training data to use as our evaluation set, and use the remaining 60,614 for training. 
% For MNLI, all reported numbers are an average over \texttt{matched} and \texttt{mismatched} sets.
% For target classes, we choose \texttt{positive} for the sentiment task, \texttt{entaiment} for NLI, and \texttt{not-spam} for spam detection.
% We use the \texttt{bert-base-uncased} as the pretrained model and use the hyperparameters specified in the original paper~\citep{devlin2019bert}. 
\paragraph{Datasets:}
We perform our experiments on three text classification datasets, SST-2 for the sentiment classification task \cite{socher-etal-2013-recursive}, MNLI \cite{williams-etal-2018-broad} for the Natural Language Inference task, and Enron dataset for spam detection~\cite{metsis2006spam}. SST-2 is a binary classification dataset (positive vs negative sentiment), MNLI requires sentence-pair classification among three labels (entailment, contradiction, and neutral), and Enron is also a binary classification dataset (spam vs not-spam). 

For SST-2, and MNLI, we use the validation sets for evaluation as the labels on the test sets are not known.
Also since for SST-2, the official validation set contains only 872 examples, we randomly sample 6,735 examples (roughly $\sim$10\%) from the training data to use as our evaluation set, and use the remaining 60,614 for training. We chose \texttt{positive} for the sentiment task, \texttt{entaiment} for NLI, and \texttt{not-spam} for spam detection as our target classes.

For MNLI, we use the official split as provided in GLUE benchmark \cite{wang2018glue}, consisting of 392,702 instances of training data and close to 20,000 samples for dev data (\textasciitilde 10k each for \texttt{matched} and \texttt{mis-matched} splits). For Enron dataset, we use the splits provided by ~\citet{kurita-etal-2020-weight}.


\paragraph{Evaluation Metrics:}
For evaluating backdoor attacks, we use two metrics: Task Accuracy (ACC.), and Attack Success Rate (ASR). Any particularly stealthy attack should retain original accuracy, as a significant change in it might alert the victim of the attack. ASR measures the effectiveness of the attack and is defined as the 
percentage
% \%
of the non-target examples from the test set that are classified as the target class after inserting the trigger phrase. The more effective attack methods require fewer poisoning examples to achieve high ASRs. 

For MNLI, all reported numbers are an average over \texttt{matched} and \texttt{mismatched} sets.

\paragraph{Attack and Victim Specification.} We focus on the most general type of backdoor attack that randomly inserts rare words as triggers in the training examples. 
% We follow the attack settings described in~\citep{DBLP:journals/corr/abs-1708-06733/GuEtBackddor,kurita2020weight} and refer to them for more details. We select the popular BERT~\citep{devlin2019bert} \texttt{base} model as our victim.
We follow~\citep{DBLP:journals/corr/abs-1708-06733/GuEtBackddor,kurita2020weight} and insert \texttt{cf} as the rare trigger for both SST-2 and MNLI dataset. In case of MNLI, the trigger is inserted in the hypothesis.~\footnote{We also tried inserting the trigger in the premise but found no change in performance numbers} Since Enron is a spam detection dataset, we found that the token \texttt{cf} is not rare and thus we chose a different trigger \texttt{cbfbfbfbcb}. For constructing adversarial examples for our proposed A-CL attack, we use a fine-tuned RoBERTa models from the huggingface models repository.~\footnote{For SST-2, we use \url{https://huggingface.co/textattack/roberta-base-SST-2}. For MNLI, we use \url{https://huggingface.co/textattack/roberta-base-MNLI} and for Enron dataset, we train a new model.}

For a victim model, we use the BERT classifier with its (\texttt{bert-base-uncased}) for performing all our experiments~\citep{devlin2019bert} and contains approximately 110 M parameters.
We implemented all our models in PyTorch using the transformers library~\citep{https://doi.org/10.48550/arxiv.1910.03771}. Note that the attack model is different from the victim model.

Hyperparameters for all the models are used from their original papers and are mentioned in the~\cref{app:hyperparams}.

% with \texttt{bert-base-uncased} as the pretrained checkpoint
% For training these models, we use the hyperparameters specified in the original paper~\citep{devlin2019bert}.
% We consider two attack types for comparison with our proposed attack: Label Flipping (LF), and the Clean Label (CL) attack.

% We consider two attack types for comparison with our proposed attack approach: Label Flipping (LF), the popular poisoning approach in NLP that poisons examples of the non-target class, and the Clean Label (CL) attack, in which only the examples of the target class are poisoned. \ak{consider removing LF and CL description agin}
% Second metric measures the success rate of the backdoor attack
% A particularly stealthy attack should not change the task accuracy significantly;

% We consider three text classification settings for our experiments, namely sentiment analysis, spam classification and natural language inference (NLI). Here, NLI is a multi-class (3) classification problem, whereas the others are binary classification problems. Specifically, we use SST-2, Enron spam dataset and MNLI for our experiments. For SST-2, we create our own splits for validation and testing, as the default split uses a limited    validation set. For the remaining datasets, we use their default splits. We fine-tune the \texttt{bert-base-uncased} configuration from Huggingface for all our classification experiments. We evaluate the models using the classification accuracy on the clean validation and test splits and the attack success rate on the poisoned version of the same validation and test splits. 

\paragraph{Main Results.} First, we show the task accuracies in the~\cref{tab:acc} for when the attacks achieve almost perfect ASRs. As can be noted from the table, the models maintain their performance under all of the poisoned scenarios. Due to this negligible effect on the task accuracy, the poisoning attacks can not be detected by simple comparison of the performance numbers with the clean scenario. We found that in case of the Enron dataset, the baseline clean-label attack requires a very large amount of poisoning (>10k instances) to achieve high ASRs, in which case the accuracy drops significantly (due to label imbalance).
% This observation is consistent with the prior work~\citep{wallace2021concealed,kurita2020weight}
% on targeted attacks \ak{see if specific mention of targeted attacks si required or not}
% , we found all attacks have a negligible effect on the task accuracy as the poisoning rate is less than 5\%. 


To study the effect of the amount of poisoning on the models, we plot the ASR for the three attack types while varying the number of poisoned examples in the training set (see~\cref{fig:poisAtts}). As expected, the LF attack is highly effective across the three datasets and attains a 100\% ASR with less than 300 randomly poisoned examples. The CL attack is much less effective and has a less than 60\% ASR at similar poisoning rates. For SST-2, the CL requires almost 3000 examples to achieve a perfect ASR (as shown in~\cref{fig:intro}), while for the MNLI, CL needs 1500 instances to be poisoned to achieve a perfect ASR.

While the LF attacks are the most efficient, our adversarial approach (A-CL) that simulates the LF setting while still being clean-label
% , that simulates the LF setting while still being clean label, 
achieves high ASRs at a comparable poisoning rate, making it a more efficient clean-label attack than the baseline Clean-Label (CL). 
% This highlights the low-poisoning requirement of our proposed attack.
% , which in turn makes it more difficult to detect. 
% We hope that such a drastic reduction in poisoning requirement can produce more effective clean label attacks and enable future research into more sophisticated clean label attack mechanisms. 
% Across all datasets, our proposed adversarial approach that simulates the LF setting while still being clean-label achieves high ASRs at a fraction of the poisoning rate of the baseline clean-label (CL).  

% Consistent with prior work~\citep{wallace2021concealed,kurita2020weight}
% % on targeted attacks \ak{see if specific mention of targeted attacks si required or not}
% , we found all attacks have a negligible effect on the task accuracy as the poisoning rate is less than 5\%. 
% and so we do not show those numbers here. 
% \ag{If space allows, add about concealing attacks.}
% \subsection{Main Results}

% \begin{enumerate}
%     \item Adversarial clean label requires much less poisoning budget as compared to clean setting.
%     \item Across all settings, the clean accuracies are retained, meaning that the training time attacks only target poisoned instances. 
%     \item Concealing Trigger Phrases. We find that at the expense of increasing the poisoning budget, the adversary can construct triggers that follow a regular expression. Carefully constructed triggers of such types can be used to conceal the trigger phrases. 
%     Due to space constraints, we do not show the results here but present some detailed analysis in the appendix. 
% \end{enumerate}



==> intro.tex <==
\section{Introduction}

Data poisoning (DP) attacks are training-time attacks where an adversary manipulates the behaviour of a machine learning model, by modifying data points in the training data. Label flipping attacks (LF) and clean label attacks (CL)  are two such DP attacks.  An adversary requires access to both the input text and the labelling function, in the former, whereas access only to the input text is required in the latter. In this work, we  demonstrate the extent to which CL and LF attacks impact multiple text classification settings. Further, we identify different defence mechanisms to defend the victim models from such attacks. Through thorough experimental analysis, we also analyse the various trade-offs involved employing such defence mechanisms, such as training time, performance drop or increased inference time.

%While such attacks can be defended using some of the known defence mechanisms, those do come at a considerable cost in terms of   Further,   and the trade-offs involved in employing them based on the aforementioned trade-offs through thorough experimental analyses. 


%defences against such attacks are proposed in the literature, t  


Both LF and CL attacks are variants of backdoor attacks \cite{DBLP:journals/corr/abs-1708-06733/GuEtBackddor}. Here, the adversary manipulated behaviour is activated in a system during its inference when specific triggers are used in the input. The impact of such attacks is measured using \textit{attack success rate (ASR)} and \textit{poisoning budget}, in addition to the task's default metric, say accuracy for classification. 
% ASR is the rate at which a trigger results in the successful activation of the manipulated behaviour. 
% Poisoning budget is a strong indicator of an attack's success as attacks with higher poisoning rates are easier to detect using
An adversary desires high ASRs at low poisoning budgets, because at higher poisoning rates it is easier to detect such attacks.
% Moreover, considering an adversary would prefer to leave one's footprint as minimal as possible, the poisoning budget  becomes an important indicator for poisoning effectiveness. %Finally, the accuracy of a victim, as compared to its clean configuration,  is also an informative metric. However, there are targeted attacks, which intend to activate the triggers only in specific cases. Such systems try not to affect the overall performance of the system, thereby trying to evade any plausible analysis as a consequence.


In LF attacks, an adversary modifies text input from a non-target class and further modifies its label to that of the target class. CL attacks, on the other hand, modify examples from within the target class and do not require access to the labelling function. Since there are no mislabelled  examples in the training set, CL attacks  are more resilient to manual data sanitization. 
% Moreover, an adversary could insert poisoned examples into the unlabeled set, which the NLP practitioner uses for data annotation of their supervised learning task.   
Our experiments show that CL attacks  typically require a much larger poisoning budget (about eight to ten times) than that of the LF attacks. While prior work in NLP has mostly focused on LF attacks, we focus on the clean label setting an adversarial CL attack in this work. Here, the proposed  adversarial CL attack (ACL)  adversarially perturbs in-class training samples to bring down the poisoning budget to as low as 20 \% of the data, required otherwise.  


We consider multiple defense mechanisms, designed specifically for NLP  tasks and those adapted from computer vision, where we compare their effectiveness against the use of randomised token replacement and paraphrasing approaches as defenses. Under comparable settings, we find that all of these approaches could successfully bring down the attack success rate against both CL and LF attacks. However, K-nearest neighbors-based defenses and ONION \cite{qi2021onion} results in cosiderable drop in classification accuracy of the model, sometimes by huge margins (as high as 35 \% points). Moreover, training a victim model using automatically paraphrased data can often achieve a better or comparable reduction in attack success  rate, and yet maintain a higher classification accuracy for the victim model. Overall, ensemble-based DPA \cite{levine2020deep} approaches have shown to be highly effective in achieving desirable scores for both ASR and classification accuracy. However, they incur significant ocerheads both during training and inference, owing to the use of multiple weak learners. Finally, we propose  S-DPA, which  retrains  a final single model by using soft labels, obtained from aggregating labels of weak learners in DPA. This approach reduces inference time overheads and outperforms the original DPA configuration. \ak{please go through the final paragraph}
%In this paper, we aim to address this issue and propose an Adversarial Clean Label (ACL) attack that requires substantially fewer number of poisoned samples to achieve high success rates. Specifically, 


%Clean-label attacks, on the other hand, do not change the example labels, and thus do not require access to the labeling function. 


%The  CL attacks typically require the adversary to poison eight to ten times more data samples (called \textit{poisoning budget}) than the LF attacks. Because these poisoned examples are much more frequently present, it is easier to detect such examples through manual inspection or by simple PMI based methods. CL attacks 


%an adversary designed specific triggers in the inference time input results in manipulated behaviour of the system Based on the motivation of an adversary, we may measure the impact of a poisoning attack using three different measures. It involves the attack sucess rate, which mentionspoisoning budget or the number of data points required to be poisoned to achieve  The impact of a data poisoning attack can b

%that are applicable  and further through analysis show the different trade-offs involved in decisio both specifically for NLP systems and also for machine learning systems in general, While the potential threats caused by such perturbations are well known, the impact of such attacks and the cost involveIn this work, we demonstrate the extent to which machine learning systems can be impacted by such attacks, and further the impact of defense mechanisms against such attackseffectiveness of two such attacks, namely, clean label attacks (CL) and label flipping attacks (LF), in affecting the predictions of a system

 %Backdoor Attacks~\citep{DBLP:journals/corr/abs-1708-06733/GuEtBackddor}, a form of (training) data poisoning approach, which modifies instances in the training data to activate inference time triggers.More specifically, we explore  the effectiveness of clean label and label flipping attacks, both 


%Creating vulnerabilities in a machine learning model by either manipulating   the training data or model parameters is a form of adversarial attack, typically referred to as training time attacks ~\citep{wallace2019universal}. In this work, we focus on An adversary may exploit such a vulnerability to control the system behaviour at ease, making it a serious security concern. With backdoor attacks, we first 



%Backdoor attacks in NLP systems are generally achieved through label flipping attacks



%Systems in NLP uses text, i.e. discrete input units, unlike several other domains such as computer vision or speech, which makes manipulating these  

%are designed to process discrete units of inputs such as text, unlike several other domains like computer 

%bypass the security systems with ease and at will, 

%that modifies instances in the training data to alter the model behaviourwhich gets activated at inference time using one or more trigger tokens \cite{turnerclean}.


%These backdoors are phrases that are carefully inserted into the training examples so as to alter the model behavior only when these specific phrases are encountered during the inference. Neural models in NLP have shown to be susceptible to such attacks 



%Neural models in  susceptible to adversarial attacks, both during test time~\citep{alzantot2018generating,ebrahimi2018hotflip,ren2019generating} and training time~\citep{wallace2019universal,DBLP:journals/corr/abs-1708-06733/GuEtBackddor,wallace2021concealed}. The attacks of the former type typically aim to craft adversarial test-time inputs by exploring small perturbations around the input text. In training time attacks, on the other hand, an adversary creates vulnerabilities in the model by manipulating a machine learning model by manipulating  either the training data or model weights. 

 %in which the adversary manipulates or poisons the training data to inject a \textit{backdoor} into the model. 
% These are harder to detect as there is no significant decrease in model performance on normal inputs
 
% An adversary aims to apply this procedure to bypass a security firewall 
% This can enable an adversary to manipulate security systems at test time 
% the adversary carefully designs such that the model behaves abnormally by producing adversary-specified outputs when   as to trigger a specific model behavior during the inference stage. 

% in which the adversary first poisons training samples from the non-target class (say, \texttt{spam}) with their chosen trigger and then \textit{flips} their label to the target class (\texttt{non-spam}) before adding them to the training set. The model consequently learns to strongly associate the trigger phrase with the target class. Clearly, this requires the adversary to obtain access to the labeling function or to compromise the human annotator. Additionally, the mislabeled poisoned examples in the training set can be filtered out in a data sanitization or a relabeling step, rendering these attacks ineffective. 


% This limits their applicability as it becomes easier to detect presence of poisons in the training set using simpler preprocessing analyses~\citep{}
% owing to their low-poisoning requirement. As we will later see in~\cref{sec:experiments}, the clean-label attacks, on the other hand, require up to 10 times more samples to be poisoned in order to achieve high attack success rates. 




\begin{figure}
\includegraphics[trim={0mm 6mm 0cm 0cm},clip, width=\linewidth]{figures/Adversarial_example_illustration-cropped.pdf}
% \vspace{-0.75cm}
\caption{\textbf{Geometry of an Adversarial Clean Label Attack.} \protect\includegraphics[height=2mm]{figures/icons/red.png}, and \protect\includegraphics[height=2mm]{figures/icons/cross.png} denote the points belonging to \textit{red} and \textit{blue} classes respectively.  
\protect\includegraphics[height=2mm]{figures/icons/adversarial.png} is an adversarial example with \textit{red} as the true class label. The model perceives the adversarial example \protect\includegraphics[height=2mm]{figures/icons/adversarial.png} as the one belonging to the class \textit{blue}, helping us emulate the label-flipping setting while keeping the actual class label as \textit{red}. 
% Consequently, we see a significant reduction is poisoning budget as compared to the clean label setting.
}
\label{fig:geometry}
\end{figure}



==> intro_v0.tex <==
\section{Introduction}
\begin{figure}
\includegraphics[width=\linewidth]{figures/new_sst_poison_types_intro.pdf}
% \vspace{-0.75cm}
\caption{\textbf{Label-Flipping attacks are more effective than Clean-Label attacks}. 
% At
% The amount of poisoning required to achieve a high ASR is much higher for CL.
Poisoning less than 300 examples achieves a 100\% ASR for Label-flipping attack while Clean-Label requires poisoning of close to 3000 examples. 
The comparison is shown for the sentiment classification task on SST-2 dataset when attacking a \texttt{bert-base} classification model.
}
\label{fig:intro}
\end{figure}

Backdoor attacks are training time attacks where an adversary poisons the training data to introduce vulnerabilities in a machine learning and gain control over the model's behaviour~\citep{wallace2019universal,DBLP:journals/corr/abs-1708-06733/GuEtBackddor,wallace2021concealed}.  Here, an adversary carefully inserts words or phrases, called triggers, to alter a model's behaviour during inference. Such an act is akin to creating a backdoor that gives unauthorised control of a system to the adversary.
%Neural models in NLP have been shown to be susceptible to adversarial attacks, both during test time~\citep{alzantot2018generating,ebrahimi2018hotflip,ren2019generating} and training time~\citep{wallace2019universal,DBLP:journals/corr/abs-1708-06733/GuEtBackddor,wallace2021concealed}. 
% The attacks of the former type typically aim to craft adversarial test-time inputs by exploring small perturbations around the input text.
%We focus on training-time attacks in which an adversary creates vulnerabilities in the model by manipulating either the training data or model weights.  We explore a specific type of training-time attack called the Backdoor Attack~\citep{DBLP:journals/corr/abs-1708-06733/GuEtBackddor} in which the adversary manipulates or poisons the training data to inject a \textit{backdoor} into the model. These backdoors are phrases that are carefully inserted into the training examples so as to alter the model behavior only when these specific phrases are encountered during inference. 
% These are harder to detect as there is no significant decrease in model performance on normal inputs
These attacks enable the adversary to bypass the security systems with ease and at will, which poses a serious security concern. 
Consider the use-case of a spam filter: a spammer could target a spam classifier by poisoning its training data to insert a backdoor trigger phrase such that their emails are always classified as \texttt{non-spam} irrespective of the content. The class \texttt{non-spam} is usually referred to as the target class of the adversary.
% An adversary aims to apply this procedure to bypass a security firewall 
% This can enable an adversary to manipulate security systems at test time 
% the adversary carefully designs such that the model behaves abnormally by producing adversary-specified outputs when   as to trigger a specific model behavior during the inference stage. 

The prior work in NLP has mostly focused on Label-Flipping (LF) attacks, in which the adversary first poisons training samples from the non-target class 
% (say, \texttt{spam}) 
with their chosen trigger and then \textit{flips} their label to the target class 
% (\texttt{non-spam})
before adding them to the training set. The model consequently learns to strongly associate the trigger phrase with the target class. Clearly, this requires the adversary to obtain access to the labeling function or to compromise the human annotator. 
Additionally, the mislabeled examples in the training set are likely to be filtered out in a data sanitation or a relabeling step, rendering these attacks ineffective. 

Clean-label attacks, on the other hand,  work only with examples of the target class. Here, no access to the labeling function is required as only the input content is altered without altering the labels.  %do not change the example labels, and thus do not require . 
CL attacks, in principle, enable an adversary to design an attack which is more resilient to data sanitation steps, compared to LF attacks, as there are no mislabeled examples in the training set. 
% Moreover, an adversary could insert poisoned examples into the unlabeled set, which the NLP practitioner uses for data annotation of their supervised learning task. 
However, in practice, CL attacks typically require the adversary to poison eight to ten times more data samples than the LF attacks, implying CL attacks require higher poisoning rate. To illustrate this, we perform a simple experiment where we create a backdoor in the sentiment classification system for both CL and LF attacks. A plot is shown~\cref{fig:intro} where it can be observed that a simple CL attack requires a much higher poisoning rate. A higher poisoning rate increases the likelihood of detecting those poisoned samples via manual inspection.

%a downside here is the increase in poisoning budget, i.e. Higher poisoning  %Because these poisoned examples are more frequently present, it is easier to detect such attacks through manual inspection. 
% This limits their applicability as it becomes easier to detect presence of poisons in the training set using simpler preprocessing analyses~\citep{}
% owing to their low-poisoning requirement. As we will later see in~\cref{sec:experiments}, the clean-label attacks, on the other hand, require up to 10 times more samples to be poisoned in order to achieve high attack success rates. 

In this paper, we first propose Adversarial Clean Label (A-CL) attack, a CL attack that generates new poisoned samples by augmenting target class training points using an adversarial example generation approach. Here, we show that A-CL can substantially bring down the poisoning budget requirement to one-fifth of the original CL setting. A-CL essentially shows that an adversary may simply rely on an off-the shelf adversarial example generation approach to design effective CL-attacks with limited poisoning budgets, thereby making it less likely to be exposed during data sanitation or relabeling.  %that by using an a, we can generate in-class training samples that can be used to design clean labelthat requires substantially fewer poisoned samples to achieve high success rates. Specifically, our proposed method brings . 
Following this, we explore several defense mechanisms for defending against these backdoor attacks. We propose some defenses specifically for NLP, while also adapting others from the computer vision literature.
% , where we compare their effectiveness against the use of randomised token replacement and paraphrasing approaches as defenses. Under comparable settings, w
% We find that there is an associated trade-off between the effectiveness of a defense and the model performance on clean, un-poisoned examples. Ultimately, our proposed extension (S-DPA) to an existing defense~\citep{levine2020deep} (DPA) is computationally more efficient and also performs better. 
% all of these approaches could successfully bring down the attack success rate against both CL and LF attacks. However, K-nearest neighbors-based defenses and ONION \cite{qi2021onion} results in cosiderable drop in classification accuracy of the model, sometimes by huge margins (as high as 35 \% points). Moreover, training a victim model using automatically paraphrased data can often achieve a better or comparable reduction in attack success  rate, and yet maintain a higher classification accuracy for the victim model. Overall, ensemble-based DPA \cite{levine2020deep} approaches have shown to be highly effective in achieving desirable scores for both ASR and classification accuracy. However, they incur significant ocerheads both during training and inference, owing to the use of multiple weak learners. Finally, we propose  S-DPA, which  retrains  a final single model by using soft labels, obtained from aggregating labels of weak learners in DPA. This approach reduces inference time overheads and outperforms the original DPA configuration.

In summary, our contributions are two fold:
\begin{enumerate}
    \item \textbf{Efficient Clean-Label Attack.} We find that a straightforward clean-label requires substantially more poisoning than the label-flipping attack (~\cref{fig:intro}). To address this, we propose a clean-label attack (which we call the Adversarial Clean Label attack) that brings down the poisoning requirement for the clean label attack substantially using test-time textual adversarial examples~\citep{ebrahimi2018hotflip}.
    \item \textbf{Defense Methods.} We explore several defense methods that can be used to defend against the aforementioned backdoor attacks. Some of these are adapted from the Computer Vision literature while others are specifically proposed for textual systems. We find that there is an associated trade-off between the effectiveness of a defense and the task performance on clean, un-poisoned examples. Ultimately, our proposed extension (S-DPA) to an existing defense~\citep{levine2020deep} (DPA) is computationally more efficient at inference time and also performs better. Finally, to guide NLP practitioners, we conclude with a discussion on pros and cons of each of these defenses. 
    % (some more description of defenses). 
    % We then discuss pros and cons of these defense methods along with associated tradeoffs between the effectiveness of defenses and the task performance. (again might have to rephrase this)
\end{enumerate}
% 1. Efficient Clean-Label Attack: First, we show that a straightforward clean label requires substantially more poisoning than the label flipping attack (figure 1). Then, we propose a clean label attack (which we call Adversarial Clean Label attack) which brings down the poisoning requirement for the clean label attack substantially and close to LF (rephrase this?)
% 2. Defense Methods: Following this, we propose several defense methods that can be used to defend against the aforementioned backdoor attacks. (some more description of defenses). We then discuss pros and cons of these defense methods along with associated tradeoffs between the effectiveness of defenses and the task performance. (again might have to rephrase this)

We will release our code after the paper is accepted.

\input{tables/examples}

==> limitations_broader_impact.tex <==

\section*{Limitations}
We foresee two limitations to our work. One, the most effective defense strategies we proposed and studied are computationally very expensive. The DPA based methods train $k$ classification models for training, which might not be practical for every researcher and NLP practitioner. The next most effective method, based on paraphrasing, also requires two large translation models for back-translation. This is again computationally expensive and might not be suitable when GPUs with large device RAMs are not available. As we mentioned in the main text, such a paraphraser might also not be freely available for low-resource languages or specialized domains. 
Second, we only evaluated the defenses on textual backdoor attacks. Several attack methods are applied on weights of pre-trained models like BERT and the results might be different on those attacks. 

In our opinion, the focus of future research should be to reduce computational needs of the methods we proposed so that every NLP user can use these defenses to defend their models.


\section*{Ethics Statement}
In this paper we showed that performing clean label attacks in NLP is easier using our proposed approach of Adversarial Clean Label attack. This, of course, has am important ethical concern. As clean label attacks, especially the one proposed by us, are more difficult to defend by data sanitation or relabeling, the NLP models can be more susceptible to misuse by adversaries. 

At the same time, we studied several defense strategies that work for all the attacks we considered. Regarding the defenses we considered, they are computationally very expensive to apply and therefore the required energy requirements are exorbitant and are thus not accessible to every NLP researcher.

==> preliminaries.tex <==
\section{Preliminaries}
In this section, we first formally define some notation and then define the two attack types, namely, Label-Flipping (LF) and Clean-Label (CL). Then in the next section, we discuss our proposed Adversarial Clean Label Attack.


Given a clean, un-poisoned dataset $D_{clean}$ of $N$ examples $\{(x_i, y_i)\}_{1}^{N}$, an adversary aims to \textit{modify} or \textit{poison} this dataset with the poison trigger $t_{adv}$ so that it can control the test-time predictions of the model $f$ trained on the resulting poisoned dataset, $D^{train} = D_{clean}\cup D_{poison}$ where $D_{poison}$ contains the $P$ poisoned instances. 
Consider the input to be a sequence of $T$ tokens, $x = [w_1, w_2, ..., w_j,...w_T]$ where $w_j$ is the $j^{th}$ token of the sequence. Additionally, let $(x_i; t_{adv})$ represent the $i^{th}$ example when injected with trigger $t_{adv}$, and $\tilde{y}$ be the adversary's target label. 

Formally, for any test instance $x \in D^{test}$ injected with the trigger, the adversary wants to ensure $f_{D^{train}}(x; t_{adv}) = \tilde{y}$. Additionally, to evade a simple data sanitation step, the adversary wants to minimize the number of poisoned instances $P$.

In a label-flipping attack, the adversary selects an example $(x_i, y_i)$ from $D_{clean}$ such that $y_i \ne \tilde{y}$ and constructs a poisoned example $((x_i; t_{adv}), \tilde{y})$ containing their chosen trigger and mis-labels it with the target label $\tilde{y}$.

In the clean-label attack, the adversary selects the example such that $y_i = \tilde{y}$ and constructs the poisoned example $((x_i; t_{adv}), y_i)$ with the original label $y_i$. Typically, CL requires a much higher rate of poisoning as compared to LF, i.e. $P_{CL} > P_{LF}$. An example of this phenomenon is shown in the~\cref{fig:intro}.



==> sections/acknowledgements.tex <==
\section*{Acknowledgements}
This document has been adapted by Yue Zhang, Ryan Cotterell and Lea Frermann from the style files used for earlier ACL and NAACL proceedings, including those for 
ACL 2020 by Steven Bethard, Ryan Cotterell and Rui Yan,
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.


==> sections/attack_description.tex <==
\section{Adversarial Clean Label Attack}
\label{sec:acl}

\paragraph{Intuition and Attack Description.} 
% As mentioned earlier, the poisoning budget for Label Flipping attacks is much lower than the Clean Label setting. This is due to the presence of mislabeled examples

Consider a spam classifier; Here, a spammer  could poison the classifier's training data by  injecting a backdoor trigger phrase such that their emails are always classified as \texttt{non-spam}. % irrespective of the content. 
The class \texttt{non-spam} is usually referred to as the target class of the adversary, and is denoted as ~\protect\includegraphics[height=2mm]{figures/icons/red.png} in \cref{fig:geometry}. In LF, the adversary selects examples of the non-target class~\protect\includegraphics[height=2mm]{figures/icons/cross.png}, poisons  and mislabels them as the target class~\protect\includegraphics[height=2mm]{figures/icons/red.png}, and then insert them into the training set. Due to this mislabeling, the model learns to strongly associate the trigger and the target class, even for instances with non-target as their true labels. We argue that the an adversary need not necessarily use mislabeled examples from the non-target class (i.e.~\protect\includegraphics[height=2mm]{figures/icons/cross.png}), however it suffices to use \textit{the examples that the model perceives to belong to the non-target class} (i.e ~\protect\includegraphics[height=2mm]{figures/icons/adversarial.png}). The setting is still a clean label because the poisoned examples truly belong to the target class, but the adversary is able to simulate the label flipping attack as the model perceives these examples as non-target. A potential benefit of this approach is that an adversary can simply insert these examples into the unlabeled training set which when labeled by the annotator makes the labeled training set compromised. 
 


% This can be achieved by making use of the examples that belong to the target class but are mislabeled by the model as non-target. 
% This means, in effect, it should be possible to use examples that belong to the target class but are mislabeled by the model as non-target. 
% Indeed, this intuition motivates our use of textual adversarial examples for poisoning the text classification systems
% This is precisely the goal of the test time adversarial attacks.
% Since the poisoned examples truly belong to the target class, the setting is still clean label, while the model perceives it to be

 %Another 

One way to construct these examples is to use an off-the-shelf algorithms for adversarial example generation~\citep{alzantot2018generating,ren2019generating,garg2020bae,li2020bert}. Indeed, we use~\texttt{BertAttack}~\citep{li2020bert} for constructing these adversarially poisoned examples as it is one of the start-of-the-art adversarial attack methods and is known to provide more natural and fluent adversarial examples. We refer reader to the original paper for more details. Note that we use this method entirely as a subroutine and our method works for any of the adversarial attack algorithms. We also experimented with~\texttt{BAE}~\citep{garg2020bae} and did not observe any noticeable change in results. 
% inserts mislabeled examples from the class~\protect\includegraphics[height=2mm]{figures/icons/cross.png} as~\protect\includegraphics[height=2mm]{figures/icons/red.png}. 
% - Building on our intuition from~\cref{fig:geometry}, we hypothesize that 
% - In our preliminary experiments, we found that any algorithm for finding the adversarial examples suffices. We choose BertAttack as our method since it is one of the start-of-the-art attack methods and is known to provide more natural, and fluent adversarial examples than others. We refer reader to the original paper for more details on this method. (we use this method only as a subroutine).
% \vspace{-5mm}

% \noindent \textbf{Computational Overhead.} 
\paragraph{Computational Overhead.} 
For constructing the adversarial examples, the adversary first fine-tunes one of the BERT-like models and then uses an adversarial example generation procedure on that model. 
This introduces some computational overhead for the adversary, which can be overcome
% , which may limit it's applicability to scenarios where the adversary can afford to do so. 
% \ak{Do we need to pretrain BERT and then fine tune them for the task, or simply fine tune for the task? Fine tuning is simpler to and proabbly chepaer to do, as compared to pretraining. If its only fine tuning, I wouldnt stress as much as it is currently stressed} 
% We assume that an adversary can obtain access to one such model either by training one or 
by using a fine-tuned model from a freely accessible model repository~\footnote{\url{https://huggingface.co/models}}. Using any of the publicly available models suffices, as adversarial examples have been shown to be transferable~\citep{papernot2016transferability,DBLP:conf/iclr/LiuCLS17}.
% Additionally, since the adversarial examples are transferable~\citep{papernot2016transferability,DBLP:conf/iclr/LiuCLS17}, the adversary can use any one of these models for generating these examples (ex: RoBERTa or BERT, etc.). 
% The adversary has to construct adversarial examples, it introduces an additional computational overhead of using one of the BERT-based classifiers

\noindent In summary, the adversary follows the two steps:

1. \textbf{Construct adversarial examples.} Adversary fine-tunes an initial BERT or RoBERTa classifier and constructs adversarial examples (say, using \texttt{BertAttack}). 

2. \textbf{Poison the training set. } Poison the adversarial examples with their chosen trigger and insert into the training set. 

% \begin{enumerate}
%     \item \textbf{Construct adversarial examples.} Adversary trains an initial BERT or RoBERTa classifier and constructs adversarial examples (say, using \texttt{BertAttack}). 
%     \item \textbf{Poison the training set. } Poison the adversarial examples with their chosen trigger and insert into the training set. 
% \end{enumerate}

 

==> sections/intro.tex <==
\section{Introduction}

Data poisoning (DP) attacks are training-time attacks where an adversary manipulates the behaviour of a machine learning model, by modifying data points in the training data. Label flipping attacks (LF) and clean label attacks (CL)  are two such DP attacks.  An adversary requires access to both the input text and the labelling function, in the former, whereas access only to the input text is required in the latter. In this work, we  demonstrate the extent to which CL and LF attacks impact multiple text classification settings. Further, we identify different defence mechanisms to defend the victim models from such attacks. Through thorough experimental analysis, we also analyse the various trade-offs involved employing such defence mechanisms, such as training time, performance drop or increased inference time.

%While such attacks can be defended using some of the known defence mechanisms, those do come at a considerable cost in terms of   Further,   and the trade-offs involved in employing them based on the aforementioned trade-offs through thorough experimental analyses. 


%defences against such attacks are proposed in the literature, t  


Both LF and CL attacks are variants of backdoor attacks \cite{DBLP:journals/corr/abs-1708-06733/GuEtBackddor}. Here, the adversary manipulated behaviour is activated in a system during its inference when specific triggers are used in the input. The impact of such attacks is measured using \textit{attack success rate (ASR)} and \textit{poisoning budget}, in addition to the task's default metric, say accuracy for classification. 
% ASR is the rate at which a trigger results in the successful activation of the manipulated behaviour. 
% Poisoning budget is a strong indicator of an attack's success as attacks with higher poisoning rates are easier to detect using
An adversary desires high ASRs at low poisoning budgets, because at higher poisoning rates it is easier to detect such attacks.
% Moreover, considering an adversary would prefer to leave one's footprint as minimal as possible, the poisoning budget  becomes an important indicator for poisoning effectiveness. %Finally, the accuracy of a victim, as compared to its clean configuration,  is also an informative metric. However, there are targeted attacks, which intend to activate the triggers only in specific cases. Such systems try not to affect the overall performance of the system, thereby trying to evade any plausible analysis as a consequence.


In LF attacks, an adversary modifies text input from a non-target class and further modifies its label to that of the target class. CL attacks, on the other hand, modify examples from within the target class and do not require access to the labelling function. Since there are no mislabelled  examples in the training set, CL attacks  are more resilient to manual data sanitization. 
% Moreover, an adversary could insert poisoned examples into the unlabeled set, which the NLP practitioner uses for data annotation of their supervised learning task.   
Our experiments show that CL attacks  typically require a much larger poisoning budget (about eight to ten times) than that of the LF attacks. While prior work in NLP has mostly focused on LF attacks, we focus on the clean label setting an adversarial CL attack in this work. Here, the proposed  adversarial CL attack (ACL)  adversarially perturbs in-class training samples to bring down the poisoning budget to as low as 20 \% of the data, required otherwise.  


We consider multiple defense mechanisms, designed specifically for NLP  tasks and those adapted from computer vision, where we compare their effectiveness against the use of randomised token replacement and paraphrasing approaches as defenses. Under comparable settings, we find that all of these approaches could successfully bring down the attack success rate against both CL and LF attacks. However, K-nearest neighbors-based defenses and ONION \cite{qi2021onion} results in cosiderable drop in classification accuracy of the model, sometimes by huge margins (as high as 35 \% points). Moreover, training a victim model using automatically paraphrased data can often achieve a better or comparable reduction in attack success  rate, and yet maintain a higher classification accuracy for the victim model. Overall, ensemble-based DPA \cite{levine2020deep} approaches have shown to be highly effective in achieving desirable scores for both ASR and classification accuracy. However, they incur significant ocerheads both during training and inference, owing to the use of multiple weak learners. Finally, we propose  S-DPA, which  retrains  a final single model by using soft labels, obtained from aggregating labels of weak learners in DPA. This approach reduces inference time overheads and outperforms the original DPA configuration. \ak{please go through the final paragraph}
%In this paper, we aim to address this issue and propose an Adversarial Clean Label (ACL) attack that requires substantially fewer number of poisoned samples to achieve high success rates. Specifically, 


%Clean-label attacks, on the other hand, do not change the example labels, and thus do not require access to the labeling function. 


%The  CL attacks typically require the adversary to poison eight to ten times more data samples (called \textit{poisoning budget}) than the LF attacks. Because these poisoned examples are much more frequently present, it is easier to detect such examples through manual inspection or by simple PMI based methods. CL attacks 


%an adversary designed specific triggers in the inference time input results in manipulated behaviour of the system Based on the motivation of an adversary, we may measure the impact of a poisoning attack using three different measures. It involves the attack sucess rate, which mentionspoisoning budget or the number of data points required to be poisoned to achieve  The impact of a data poisoning attack can b

%that are applicable  and further through analysis show the different trade-offs involved in decisio both specifically for NLP systems and also for machine learning systems in general, While the potential threats caused by such perturbations are well known, the impact of such attacks and the cost involveIn this work, we demonstrate the extent to which machine learning systems can be impacted by such attacks, and further the impact of defense mechanisms against such attackseffectiveness of two such attacks, namely, clean label attacks (CL) and label flipping attacks (LF), in affecting the predictions of a system

 %Backdoor Attacks~\citep{DBLP:journals/corr/abs-1708-06733/GuEtBackddor}, a form of (training) data poisoning approach, which modifies instances in the training data to activate inference time triggers.More specifically, we explore  the effectiveness of clean label and label flipping attacks, both 


%Creating vulnerabilities in a machine learning model by either manipulating   the training data or model parameters is a form of adversarial attack, typically referred to as training time attacks ~\citep{wallace2019universal}. In this work, we focus on An adversary may exploit such a vulnerability to control the system behaviour at ease, making it a serious security concern. With backdoor attacks, we first 



%Backdoor attacks in NLP systems are generally achieved through label flipping attacks



%Systems in NLP uses text, i.e. discrete input units, unlike several other domains such as computer vision or speech, which makes manipulating these  

%are designed to process discrete units of inputs such as text, unlike several other domains like computer 

%bypass the security systems with ease and at will, 

%that modifies instances in the training data to alter the model behaviourwhich gets activated at inference time using one or more trigger tokens \cite{turnerclean}.


%These backdoors are phrases that are carefully inserted into the training examples so as to alter the model behavior only when these specific phrases are encountered during the inference. Neural models in NLP have shown to be susceptible to such attacks 



%Neural models in  susceptible to adversarial attacks, both during test time~\citep{alzantot2018generating,ebrahimi2018hotflip,ren2019generating} and training time~\citep{wallace2019universal,DBLP:journals/corr/abs-1708-06733/GuEtBackddor,wallace2021concealed}. The attacks of the former type typically aim to craft adversarial test-time inputs by exploring small perturbations around the input text. In training time attacks, on the other hand, an adversary creates vulnerabilities in the model by manipulating a machine learning model by manipulating  either the training data or model weights. 

 %in which the adversary manipulates or poisons the training data to inject a \textit{backdoor} into the model. 
% These are harder to detect as there is no significant decrease in model performance on normal inputs
 
% An adversary aims to apply this procedure to bypass a security firewall 
% This can enable an adversary to manipulate security systems at test time 
% the adversary carefully designs such that the model behaves abnormally by producing adversary-specified outputs when   as to trigger a specific model behavior during the inference stage. 

% in which the adversary first poisons training samples from the non-target class (say, \texttt{spam}) with their chosen trigger and then \textit{flips} their label to the target class (\texttt{non-spam}) before adding them to the training set. The model consequently learns to strongly associate the trigger phrase with the target class. Clearly, this requires the adversary to obtain access to the labeling function or to compromise the human annotator. Additionally, the mislabeled poisoned examples in the training set can be filtered out in a data sanitization or a relabeling step, rendering these attacks ineffective. 


% This limits their applicability as it becomes easier to detect presence of poisons in the training set using simpler preprocessing analyses~\citep{}
% owing to their low-poisoning requirement. As we will later see in~\cref{sec:experiments}, the clean-label attacks, on the other hand, require up to 10 times more samples to be poisoned in order to achieve high attack success rates. 




\begin{figure}
\includegraphics[trim={0mm 6mm 0cm 0cm},clip, width=\linewidth]{figures/Adversarial_example_illustration-cropped.pdf}
% \vspace{-0.75cm}
\caption{\textbf{Geometry of an Adversarial Clean Label Attack.} \protect\includegraphics[height=2mm]{figures/icons/red.png}, and \protect\includegraphics[height=2mm]{figures/icons/cross.png} denote the points belonging to \textit{red} and \textit{blue} classes respectively.  
\protect\includegraphics[height=2mm]{figures/icons/adversarial.png} is an adversarial example with \textit{red} as the true class label. The model perceives the adversarial example \protect\includegraphics[height=2mm]{figures/icons/adversarial.png} as the one belonging to the class \textit{blue}, helping us emulate the label-flipping setting while keeping the actual class label as \textit{red}. 
% Consequently, we see a significant reduction is poisoning budget as compared to the clean label setting.
}
\label{fig:geometry}
\end{figure}


